From Individual to Society: A Survey on Social Simulation Driven by Large Language Model-based Agents

Traditional sociological research often relies on human participation, which, though effective, is expensive, challenging to scale, and with ethical concerns. Recent advancements in large language models (LLMs) highlight their potential to simulate human behavior, enabling the replication of individual responses and facilitating studies on many interdisciplinary studies. In this paper, we conduct a comprehensive survey of this field, illustrating the recent progress in simulation driven by LLM-empowered agents. We categorize the simulations into three types: (1) Individual Simulation, which mimics specific individuals or demographic groups; (2) Scenario Simulation, where multiple agents collaborate to achieve goals within specific contexts; and (3) Society Simulation, which models interactions within agent societies to reflect the complexity and variety of real-world dynamics. These simulations follow a progression, ranging from detailed individual modeling to large-scale societal phenomena. We provide a detailed discussion of each simulation type, including the architecture or key components of the simulation, the classification of objectives or scenarios and the evaluation method. Afterward, we summarize commonly used datasets and benchmarks. Finally, we discuss the trends across these three types of simulation. A repository for the related sources is at {\url{https://github.com/FudanDISC/SocialAgent}}.

==> tabs/indi_tab.tex <==
\begin{table*}[!htp]
	\aboverulesep0pt
	\belowrulesep0pt
	\extrarowheight1pt
	\centering
	\footnotesize
	\tabcolsep3pt
	\begin{tabularx}{\linewidth}{c|>{\centering\arraybackslash}X|c|c|c|c|>{\centering\arraybackslash}m{8em}}
		\toprule
        \multirow[m]{2}{*}{\textbf{Objectives}} 
		& \multirow[m]{2.5}{2.5em}{\textbf{Paper}} & \multicolumn{4}{c|}{\textbf{Aritecture}} & \multirow[m]{2.5}{*}{\textbf{Construtction}} \\
		\cmidrule{3-6}
		&  & \textbf{Profile} & \textbf{Memory} & \textbf{Planning} & \textbf{Action Domain} &  \\
		\midrule
		\multirow[m]{19}{*}{\textbf{Characters}} & \cite{brahman2021letcharacterstellstory} & Dialogue/Description & Short-term & - & Open/Closed  & Parametric  \\
		\cmidrule{2-7}
		& \cite{chen2023largelanguagemodelsmeet} & Dialogue/Description & Short-term & - & Open  & \multicolumn{1}{m{7em}}{Parametric /Nonparametric }\\
		\cmidrule{2-7}
		& \cite{schwitzgebel2023creatinglargelanguagemodel} & Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{park2023generativeagentsinteractivesimulacra} & Description & Short/Long-term & Interactive & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{agrawal-etal-2023-multimodal} & Dialogue/Description & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{li2023chatharuhirevivinganimecharacter} & Dialogue & Short-term & Isolated & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{gao2023livechatlargescalepersonalizeddialogue} & Dialogue/Description & Short/Long-term & - & Open/Closed  & Parametric  \\
		\cmidrule{2-7}
		& \cite{wang2024rolellmbenchmarkingelicitingenhancing} & Description/Dialogue & Short-term & - & Open/Closed  & Parametric  \\
		\cmidrule{2-7}
		& \cite{shao2023characterllmtrainableagentroleplaying} & Description & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{wang2024incharacterevaluatingpersonalityfidelity} & - & Short-term & - & Open/Closed  & - \\
		\cmidrule{2-7}
		& \cite{zhou2023characterglmcustomizingchineseconversational} & Description/Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{shen2024roleevalbilingualroleevaluation} & Description & Short-term & - & Closed  & Parametric  \\
		\cmidrule{2-7}
		& \cite{tu2024characterevalchinesebenchmarkroleplaying} & Dialogue & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{yu2024neekoleveragingdynamiclora} & Description & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{xu2024characterdestinylargelanguage} & Description & Short/Long-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{yuan2024evaluatingcharacterunderstandinglarge} & Description & Short-term & - & Open/Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{ran2024capturingmindsjustwords} & Description/Dialogue & Short/Long-term & - & Open/Closed  & Parametric  \\
		\cmidrule{2-7}
		& \cite{dai2024mmrolecomprehensiveframeworkdeveloping} & Description & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{yu2024dialogueprofiledialoguealignmentframework} & Dialogue & Short-term & - & Open  & Parametric  \\
		\midrule
		 \multirow[m]{35}{6em}{\textbf{Demographics}}& \cite{karra2023estimatingpersonalitywhiteboxlanguage} & Dialogue/Description & Short-term & - & Closed  & Parametric  \\
		 \cmidrule{2-7}
		& \cite{jiang2023evaluatinginducingpersonalitypretrained} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{Liu_2022} & Description & Short/Long-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{Argyle_2023} & Description & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{horton2023largelanguagemodelssimulated} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{xie2023wallstreetneophytezeroshot} & Description & Short-term & Isolated & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{deshpande2023toxicitychatgptanalyzingpersonaassigned} & Description & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{xiang2023languagemodelsmeetworld} & Description & Short-term & Interactive & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{song2023largelanguagemodelsdeveloped} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{cheng2023markedpersonasusingnatural} & Description & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{wang2024userbehaviorsimulationlarge} & Description & Short/Long-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{serapiogarcía2023personalitytraitslargelanguage} & Description & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{huang2024emotionallynumbempatheticevaluating} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{tu2023characterchatlearningconversationalai} & Description & Short/Long-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{abbasian2024conversationalhealthagentspersonalized} & Description & Short/Long-term & Interactive & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{chen2024moneymouthisevaluating} & Description & Short/Long-term & Interactive & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{li2024econagentlargelanguagemodelempowered} & Description & Short/Long-term & - & Open  & Nonparamaetric  \\
		\cmidrule{2-7}
		& \cite{shea2023buildingpersonaconsistentdialogue} & Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{chawla2023selfishwiselyinvestigatingimpact} & Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{10.19066/COGSCI.2024.35.1.002} & - & Short-term & Interactive & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{gupta2024biasrunsdeepimplicit} & Description & Short-term & - & Open  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{li2024steerabilitylargelanguagemodels} & Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{huang2024embodiedgeneralistagent3d} & Description & Short-term & Isolated & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{xie2024largelanguagemodelagents} & Description & Short-term &  & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{Lee_2024} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{li2024culturellmincorporatingculturaldifferences} & Dialogue & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{weng2024controllmcraftingdiversepersonalities} & - & Short/Long-term & - & Open  & Nonparamatric  \\
		\cmidrule{2-7}
		& \cite{sun2024randomsiliconsamplingsimulating} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{Bisbee_Clinton_Dorff_Kenkel_Larson_2024} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{ge2024scalingsyntheticdatacreation} & Description & Short-term & - & Open  & Parametric  \\
		\cmidrule{2-7}
		& \cite{Qu2024PerformanceAB} & Description & Short-term & - & Closed  & Nonparametric  \\
		\cmidrule{2-7}
		& \cite{qiu2024interactiveagentssimulatingcounselorclient} & Description & Short-term & - & Open  & Nonparametric  \\
		\bottomrule
	\end{tabularx}
    \caption{A list of representative works of individual simulation}
\end{table*}


